ComDrive: Comfort-Oriented End-to-End Autonomous Driving

We propose ComDrive: the first comfort-oriented end-to-end autonomous driving system to generate temporally consistent and comfortable trajectories. Recent studies have demonstrated that imitation learning-based planners and learning-based trajectory scorers can effectively generate and select safety trajectories that closely mimic expert demonstrations. However, such trajectory planners and scorers face the challenge of generating temporally inconsistent and uncomfortable trajectories. To address these issues, ComDrive first extracts 3D spatial representations through sparse perception, which then serves as conditional inputs. These inputs are used by a Conditional Denoising Diffusion Probabilistic Model (DDPM)-based motion planner to generate temporally consistent multi-modal trajectories. A dual-stream adaptive trajectory scorer subsequently selects the most comfortable trajectory from these candidates to control the vehicle. Experiments demonstrate that ComDrive achieves state-of-the-art performance in both comfort and safety, outperforming UniAD by 17% in driving comfort and reducing collision rates by 25% compared to SparseDrive. More results are available on our project page: https://jmwang0117.github.io/ComDrive/.

==> Tables/ablation_motion_planner.tex <==
\begin{table}[t]
  \centering
  
  \caption{Ablation for designs in parallel motion planner. "HPT" denotes the incorporation of historical prediction trajectory into the DDPM; "H-S\&A" represents the inclusion of historical trajectory speed and acceleration in the DDPM; "RTS" refers to the utilization of a rule-based scoring system for planning purposes; "VTS" signifies the employment of a Llama 3.2V; "FTS" indicates the use of a Fixed Trajectory Set instead of DDPM.}
  \label{tab:ablation_motion_planner}
  \vspace{5pt}
  \scriptsize
  \setlength{\tabcolsep}{1.0mm}
  \begin{tabular}{ccccc|cccc|cccc}
    \toprule
    \multirow{2}{*}{HPT} & 
    \multirow{2}{*}{H-S\&A} &
    \multirow{2}{*}{RTS} & 
    \multirow{2}{*}{VTS} &
    \multirow{2}{*}{FTS} &
    \multicolumn{4}{c|}{Planning L2($m$)} & 
    \multicolumn{4}{c}{Planning Coll.(\%)} \\
    & & & & & 1$s$ & 2$s$ & 3$s$ & \cellcolor{gray!20}Avg. & 1$s$ & 2$s$ & 3$s$ & \cellcolor{gray!20}Avg.\\
    \midrule
    \checkmark & \checkmark & \checkmark & \checkmark & & \textbf{0.31} & \textbf{0.58} & \textbf{0.93} & \cellcolor{gray!20}\textbf{0.60} & \textbf{0.01} & \textbf{0.05} & \textbf{0.16} & \cellcolor{gray!20}\textbf{0.07} \\
    \checkmark & \checkmark & \checkmark & & & 0.41 & 0.83 & 1.21 & \cellcolor{gray!20}0.81 & 0.02 & 0.13 & 0.58 & \cellcolor{gray!20}0.24 \\
    \checkmark & & \checkmark & \checkmark & & 0.34 & 0.67 & 1.11 & \cellcolor{gray!20}0.71 & 0.03 & 0.09 & 0.20 & \cellcolor{gray!20}0.11 \\
    & \checkmark & \checkmark & \checkmark & & 0.37 & 0.71 & 1.19 & \cellcolor{gray!20}0.76 & 0.03 & 0.11 & 0.61 & \cellcolor{gray!20}0.25\\
    & & \checkmark & \checkmark & \checkmark & 0.45 & 0.92 & 1.38 & \cellcolor{gray!20}0.92 & 0.04 & 0.15 & 0.72 & \cellcolor{gray!20}0.30 \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables/navisim_result.tex <==
\definecolor{Gray}{gray}{0.85} % 定义颜色
\begin{table*}[htp]

\centering % 表格居中
\caption{\textbf{Performance on the OpenScene dataset.} NC, DAC, TTC, C, EP correspond to No at-fault Collisions, Drivable Area Compliance, Time to Collision, Comfort, and Ego Progress, respectively.} 
\label{table:result}

\begin{tabular}{l|ccccc|c}
    \toprule
    Method 
    & NC 
    & DAC
    & EP 
    & TTC 
    & C 
    & Score  \\
    \midrule
    Transfuser~\cite{chitta2022transfuser}  & 96.5 & 87.9 & 73.9 & 90.2 & 100 & 78.0  \\
    Vadv2-$\mathcal{V}_{4096}$~\cite{chen2024vadv2} & 97.1 & 88.8 & 74.9 & 91.4 & 100 & 79.7   \\
    Vadv2-$\mathcal{V}_{8192}$~\cite{chen2024vadv2} & 97.2 & 89.1 & 76.0 & 91.6 & 100 & 80.9   \\
    HyDra-MDP-$\mathcal{V}_{4096}$~\cite{li2024hydra}    & 97.7 & 91.5 & 77.5 & 92.7 & 100 & 82.6 \\
    HyDra-MDP-$\mathcal{V}_{8192}$~\cite{li2024hydra}    & 97.9 & 91.7 & 77.6 & 92.9 & 100 & 83.0 \\
    \midrule
    ComDrive (ours)  & \cellcolor{Gray}\textbf{98.4} & \cellcolor{Gray}\textbf{92.1} & \cellcolor{Gray}\textbf{78.9} & \cellcolor{Gray}\textbf{96.7} & \cellcolor{Gray}\textbf{100} & \cellcolor{Gray}\textbf{85.2} \\
\bottomrule
\end{tabular}
\vspace{-2mm} % 调整表格下方空间
\end{table*}

